Some Unipotent Arthur Packets for Reductive $p$-adic Groups

Let $k$ be a $p$-adic field and let $\mathbf{G}(k)$ be the $k$-points of a connected reductive group, inner to split. The set of Aubert-Zelevinsky duals of the constituents of a tempered L-packet form an Arthur packet for $\mathbf{G}(k)$. In this paper, we give an alternative characterization of such Arthur packets in terms of the wavefront set, proving in some instances a conjecture of Jiang-Liu and Shahidi. Pursuing an analogy with real and complex groups, we define some special unions of Arthur packets which we call \emph{weak} Arthur packets and describe their constituents in terms of their Langlands parameters.

==> scraps.tex <==




\section{Introduction}

Let $\mathsf k$ be a nonarchimedean local field of characteristic $0$ with ring of integers $\mathfrak o$, finite residue field $\mathbb F_q$ of cardinality $q$ and valuation $\mathsf{val}_{\mathsf k}$. Fix an algebraic closure $\bar{\mathsf k}$ of $\mathsf k$ and let $K\subset \bar{\mathsf k}$ be the maximal unramified extension of $\mathsf k$ in $\bar{\mathsf k}$. Let $\mathbf{G}$ be a connected reductive algebraic group defined over $\sfk$ and let $\mathbf{G}(\sfk)$ be the group of $\sfk$-rational points. We assume throughout that $\mathbf{G}(\sfk)$ is inner to split. 

Let $W_{\sfk}$ be the Weil group associated to $\sfk$ \cite[(1.4)]{Tate1979}. Then the Weil-Deligne group is the semidirect product \cite[\S 8.3.6]{Deligne1972}
%
$$W_{\sfk}' = W_k \rtimes \CC$$
%
where $W_k$ acts on $\CC$ via
%
$$w x w^{-1}=\|w\| x,\qquad x\in \mathbb C,\ w\in W_k.$$
%
Let $G^{\vee}$ denote the complex Langlands dual group associated to $\mathbf{G}$, see \cite[\S2.1]{Borel1979}. 

\begin{definition}\label{def:Langlandsparams}
A \emph{Langlands parameter} is a continuous homomorphism
%
\begin{equation}
    \phi: W_k'\rightarrow G^\vee
\end{equation}
%
which respects the Jordan decompositions in $W_k'$ and $G^\vee$ (\cite[\S8.1]{Borel1979}). We say that $\phi$ is \emph{unramified} if it is trivial when restricted to the inertia subgroup $I_k$ of $W_k$.
\end{definition}

If we fix a generator $\mathsf{Fr}$ of the infinite cyclic group $W_k/I_k$, we get a bijection between the set of unramified Langlands parameters and pairs of the form
%
\begin{equation}\label{e:unramified-Langlands}
   (s,u) \in G^{\vee} \times G^{\vee},\qquad s\text{ semisimple},\ u \text{ unipotent}, \ sus^{-1}=u^q.
\end{equation}
%
This bijection is defined by $\phi \mapsto (s,u) = (\phi(\mathsf{Fr}),\phi(1))$, where $1\in\mathbb{C}\subset W'_k$. Replacing $u$ with $n \in \fg^{\vee}$ such that $q^n=u$, we get a further bijection onto pairs of the form
%
\begin{equation}\label{e:unramified-Langlands2}(s, n) \in G^{\vee} \times \fg^{\vee}, \qquad s\text{ semisimple},\ n \text{ nilpotent}, \ \Ad(s)n=qn.\end{equation}
%
To each Langlands parameter $\phi$, one hopes to associate an $L$-packet $\Pi^{\mathsf{Lan}}_{\phi}(\mathbf{G}(k))$ of irreducible admissible $\mathbf{G}(k)$-representations \cite[\S10]{Borel1979}. For unramified parameters, the $L$-packets were defined by ?? in ??. If $\phi$ is an unramified Langlands parameter which corresponds to the pair $(s,n)$, the $L$-packet $\Pi_{\phi}^{\mathsf{Lan}}(\mathbf{G}(k))$ is parameterized by the set of irreducible representations of the component group $A(s,n)$ of the mutual centralizer in $G^\vee$ of $s$ and $n$, such that the center $Z(G^\vee)$ acts trivially on $\rho$\todo{inner to split}. This is known as the Deline-Langlands-Lusztig correspondence, see Theorem \ref{thm:Langlands} below.

%Let us return to the general setting of Definition \ref{def:Langlandsparams}. 
Of fundamental importance are the \emph{tempered} Langlands parameters. If $k$ is Archimedean, a Langlands parameter is tempered if the image of $W_k$ is bounded. If $k$ is non-Archimedean, the definition of `tempered' is more subtle in general. For unramified parameters, `tempered' means that the semisimple element $s$ in (\ref{e:unramified-Langlands}) is `relatively compact', see Theorem \ref{thm:Langlands}(1) for a more precise condition.




\subsection{Unipotent representations: wavefront sets}\label{sec:results}



Our main results concern the set of representations with \emph{unipotent cuspidal support} introduced by Lusztig \cite{Lu-unip1} (see Section \ref{s:unip-cusp} for the precise definition). In terms of the Langlands correspondence, see Section \ref{sec:Arthur}, these are exactly the representations which correspond to unramified Langlands parameters. Recall that the set of unramified Langlands parameters is in bijection pairs $(s,n)$ of the form described in (\ref{e:unramified-Langlands2}), and the $L$-packet corresponding to the pair $(s,n)$ is in bijection with irreducible representations $\rho$ of $A(s,n)$ on which the center $Z(G^{\vee})$ acts trivially. Hence, the set of irreducible representations with unipotent cuspidal support is in bijection with $G^{\vee}$-conjugacy classes of triples $(s,n,\rho)$. Write $X(s,n,\rho)$ for the irreducible representation corresponding to $(s,n,\rho)$. Since triples are considered up to conjugation by $G^{\vee}$, we may assume without loss of generality that $s$ belongs to a fixed maximal torus $T^\vee$ of $G^\vee$. There is a polar decomposition 
\[T^\vee=T_c^\vee T_{\mathbb R}^\vee
\]
where $T^{\vee}_c$ is compact and $T^{\vee}_{\RR}$ is a vector group, see (\ref{eq:real}). We say that $s$ is \emph{real} if $s\in T^\vee_{\mathbb R}$, and in this case, we say that $X(s,n,\rho)$ has \emph{real infinitesimal character}. 

As is well-known, the category of smooth $\bfG(\mathsf k)$-representation decomposes as a product of full subcategories, called \emph{Bernstein blocks}, see \cite[(2.10)]{Bernstein1984}. The category of representations with unipotent cuspidal support is a finite product of Bernstein blocks. The block containing the trivial representation (known as the \emph{principal block}) is precisely the category of \emph{Iwahori-spherical representations} (i.e. smooth representations generated by their Iwahori-fixed vectors). Under the Deligne-Langlands-Lusztig correspondence, the irreducible Iwahori-spherical representations correspond to the triples $(s,n,\rho)$ for which $\rho$ is of \emph{Springer type}. This means that $\rho$ occurs in the permutation representation of $A(s,n)$ in the top cohomology group of the variety of Borel subalgebras of $\mathfrak g^\vee$ that contain $n$ and are invariant under $\mathrm{Ad}(s)$. Notably, the set of irreducible representations with unipotent cuspidal support is the smallest class of representations which is a union of $L$-packets and contains all Iwahori-spherical representations, see Theorem \ref{thm:Langlands}.

An important role will be played by the \emph{Aubert-Zelevinsky} involution \cite{Au}, denoted $X \mapsto \mathrm{AZ}(X)$, see Section \ref{sec:AZduality}. This is an involution on the Grothendieck group of finite-length smooth $\mathbf{G}(\sfk)$-representations which preserves  the Grothendieck group of each Bernstein block and carries irreducibles to irreducibles (up to a sign). In the case of representations with unipotent cuspidal support, it preserves the semisimple parameter $s$. For example, $\mathrm{AZ}$ takes the trivial representation to the Steinberg discrete series representation, and more generally, a spherical representation to the unique generic representation (in the sense of admitting Whittaker models) with the same semisimple parameter. 

A fundamental invariant attached to an admissible representation $X$ is its \emph{wavefront set}. In its classical form, the wavefront set $\WF(X)$ of $X$ is a collection of nilpotent $\bfG(\sfk)$-orbits in the Lie algebra $\mathfrak g(\sfk)$: these are the maximal orbits for which the Fourier transforms of the corresponding orbital integrals contribute to the Harish-Chandra-Howe local character expansion of the distribution character of $X$, \cite[Theorem 16.2]{HarishChandra1999}. In this paper, we consider two coarser invariants (see Section \ref{s:wave} for the precise definitions). The first of these invariants is the \emph{algebraic wavefront set}, denoted $\hphantom{ }^{\bar{\sfk}}\WF(X)$. This is a collection of nilpotent orbits in $\mathfrak{g}(\bark)$, see for example \cite[p. 1108]{Wald18} (where it is simply referred to as the `wavefront set' of $X$). The second invariant is a natural refinement $^K\WF(X)$ of $\hphantom{ }^{\bar{\sfk}}\WF(X)$ called the \emph{canonical unramified wavefront set}, defined recently in \cite{okada2021wavefront}. This is a collection of nilpotent orbits $\mathfrak g(K)$ (modulo a certain equivalence relation $\sim_A$). The relationship between these three invariants is as follows: the algebraic wavefront set $\hphantom{ }^{\bar{\sfk}}\WF(X)$ is deducible from the usual wavefront set $\WF(X)$ as well as the canonical unramified wavefront set $^K\WF(X)$. It is not known whether the canonical unramified wavefront set is deducible from the usual wavefront set, but we expect this to be the case, see \cite[Section 5.1]{okada2021wavefront} for a careful discussion of this topic. 

The final ingredient that we need in order to state our main result on wavefront sets is a refinement $D$ due to Achar \cite{Acharduality} of the duality map $d$. Suppose $G$ is the complex reductive group with dual $G^\vee$. Let $\mathcal N_{o,\bar c}$ be the set of pairs $(\mathbb O,\bar C)$ consisting of a nilpotent orbit $\mathbb O\in \mathcal N_o$ and a conjugacy class $\bar C$ in $\bar A(\mathbb O)$, Lusztig's canonical quotient of the $G$-equivariant fundamental group $A(\OO)$ of $\OO$. Let $\mathcal N^\vee_{o,\bar{c}}$ be the corresponding set for $G^\vee$. The duality $D$ is a map
\[D: \mathcal N^\vee_{o,\bar c}\rightarrow \mathcal N_{o,\bar c}
\]
satisfying certain properties, see section \ref{subsec:nilpotent}. One of these properties is:
\[D(\OO^\vee,1)=(d(\OO^\vee),\bar C'),
\]
where $\bar{C}'$ is a conjugacy class in $\bar{A}(d(\OO^{\vee}))$ (which is trivial in the case when $\OO^\vee$ is special in the sense of Lusztig).

In \cite[Section 5.1]{okada2021wavefront}, it is shown that there is canonical bijection between $\mathcal N_{o,\bar c}$ and the set of $\sim_A$-classes of unramified nilpotent orbits $\mathcal N_o(K)$ of $\bfG(K)$. This is recalled in section \ref{subsec:nilpotent}. This way, we can think of $D(\OO^\vee, \bar{C})$ as a class in $\mathcal N_o(K)/\sim_A$.

%Our first main result is the following (note the analogy with Theorem \ref{thm:WFBV}).

\begin{theorem}[See Theorems \ref{thm:realwf}, \ref{cor:wfbound} below]\label{t:main} Let $X=X(s,n,\rho)$ be an irreducible smooth Iwahori-spherical $\bfG(\mathsf k)$-representation with real infinitesimal character and let $\AZ(X) = X(s,n',\rho')$. 
%Suppose in addition that $s'$ is real, in the sense of Remark \ref{r:real}. 
\begin{enumerate}
    \item The canonical unramified wavefront set $^K\WF(X)$ is a singleton, and
\[^K\WF(X) = D(\OO^{\vee}_{\AZ(X)},1),\]
where $\OO^{\vee}_{\AZ(X)}$ is the $G^\vee$-orbit of $n'$ and $D$ is the duality map defined by Achar. In particular,
\[\hphantom{ }^{\bar{\sfk}}\WF(X) = d(\OO^\vee_{\AZ(X)}).\]
\item Suppose $X=X(q^{\frac 12 h^\vee},n,\rho)$ where $h^\vee$ is the neutral element of a Lie triple attached to a nilpotent orbit $\OO^\vee\subset \mathfrak g^\vee$. Then
\[D(\OO^{\vee}, 1) \leq_A \hphantom{ } ^K\WF(X),
\]
%
where $\leq_A$ is the partial order defined by Achar. In particular,
\[d(\OO^{\vee}) \le \hphantom{ }^{\bar{\sfk}}\WF(X).\]
\end{enumerate}
\end{theorem}





\subsection{Arthur's conjectures}\label{sec:Arthur}
Theorem \ref{t:main} fits into the framework of \cite{AdamsBarbaschVogan} for defining the most basic Arthur packets.
 We begin by recalling some of the local implications of Arthur's conjectures about automorphic forms \cite{Arthur1983,Arthur1989}.


\begin{definition}%[Section 6, \cite{Arthur1989}]
An \emph{Arthur parameter} is a continuous homomorphism
%
$$\psi: W_k' \times \mathrm{SL}(2,\CC) \to G^{\vee}$$
%
such that
\begin{itemize}
    \item[(i)]  The restriction of $\psi$ to $W_k'$ is a tempered Langlands parameter.
       \item[(ii)] The restriction of $\psi$ to $\mathrm{SL}(2,\CC)$ is algebraic.
\end{itemize}
Arthur parameters are considered modulo the $G^{\vee}$-action on the target.
\end{definition}



For each Arthur parameter $\psi$ there is an associated Langlands parameter $\phi_{\psi}: W_k' \to G^{\vee}$ defined by the formula
%
\begin{equation}\label{eq:ArthurLanglands}\phi_{\psi}(w) = \psi(w,\begin{pmatrix}\|w\|^{1/2} & 0\\0 & \|w\|^{-1/2} \end{pmatrix}), \qquad w \in W_k',\end{equation}
%
where $\|\bullet\|$ is the pull-back to $W_k'$ of the norm map on $W_k$. (Note: this is \emph{not} merely the restriction $\psi|_{W_k'}$, which is also a Langlands parameter.)  The local version of Arthur's conjectures can be stated succinctly as follows.

\begin{conj}[Section 6, \cite{Arthur1989}]\label{conj:Arthur}
For each Arthur parameter $\psi$, there is an associated finite set $\Pi_{\psi}^{\mathsf{Art}}(\mathbf{G}(k))$ of irreducible admissible $\mathbf{G}(k)$-representations  called the \emph{Arthur packet} attached to $\psi$. The set $\Pi_{\psi}^{\mathsf{Art}}(\mathbf{G}(k))$ should satisfy various properties, including:
\begin{itemize}
    \item[(i)] $\Pi^{\mathsf{Lan}}_{\phi_{\psi}}(\mathbf{G}(k)) \subseteq \Pi_{\psi}^{\mathsf{Art}}(\mathbf{G}(k))$,
    \item[(ii)] $\Pi_{\psi}^{\mathsf{Art}}(\mathbf{G}(k))$ consists of unitary representations,
    %\item[(iii)] The elements of $\Pi_{\psi}^{\mathsf{Art}}(\mathbf{G}(k))$ are parameterized by irreducible representations of a finite group $A_{\psi}$ which is recovered in a natural fashion from $\psi$.
\end{itemize}
along with several other properties (e.g. stability, endoscopy), see \cite[Section 4]{Arthur1989} or \cite[Chapter 1]{AdamsBarbaschVogan}.
\end{conj}

Note that if $\psi$ is trivial on the $\mathrm{SL}(2,\CC)$ factor, then $\phi_{\psi} = \psi|_{W_k'}$, a tempered Langlands parameter. In this case, the inclusion $\Pi^{\mathsf{Lan}}_{\phi_{\psi}}(\mathbf{G}(k)) \subseteq \Pi^{\mathsf{Art}}_{\psi}(\mathbf{G}(k))$ is an equality. Thus, tempered $L$-packets are also Arthur packets.

Let us briefly summarize the status of Arthur's conjectures. For $k \in \{\RR,\CC\}$, the packets $\Pi_{\psi}^{\mathsf{Art}}(\mathbf{G}(k))$ were defined in \cite[Chapter 22]{AdamsBarbaschVogan} using microlocal geometry (the packets they propose are shown to satisfy all of Arthur's properties, except for unitarity, which remains an open question).  For quasisplit classical groups (orthogonal and symplectic) and any local field $k$, Arthur defined the packets $\Pi_{\psi}^{\mathsf{Art}}(\mathbf{G}(k))$ using endoscopic transfer and proved that they satisfy all of the conjectured properties \cite[Theorems 1.5.1 and 2.2.1]{Arthur2013}. Arthur's constructions have been extended to quasisplit unitary groups in \cite{Mok2015}. For $k$ a $p$-adic field, there is, as of yet, no general definition of $\Pi_{\psi}^{\mathsf{Art}}(\mathbf{G}(k))$, although the problem of producing one has generated a substantial body of research. For classical $p$-adic groups, explicit definitions, compatible with Arthur's,  were proposed by M\oe glin in \cite{Mo1,Mo2}, see also the exposition in \cite{Xu} and the references therein. For $p$-adic $G_2$, some (non-tempered) Arthur packets were constructed in \cite{GanGurevich}. Recently, Cunningham et. al. have proposed a `microlocal' approach to defining Arthur packets, see \cite{Cunningham}. 

The wavefront set results allow us to propose a new definition of the Arthur packets associated to a particular class of Arthur parameters. The parameters we consider are `as far from tempered as possible'. This means that the restrictions $\psi|_{W_k'}$ are `as close to trivial as possible'. 

\begin{definition}\label{def:unipotentparam}
An Arthur parameter $\psi$ is \emph{anti-tempered} if the restriction $\psi|_{W_k'}$ is trivial. 
\end{definition}

In \cite{Arthur1989}, Arthur introduced the notion of a \emph{unipotent Arthur parameter}, although he did not provide a precise definition (except over $\RR$). Certainly, all of the parameters included in Definition \ref{def:unipotentparam} deserve to be called unipotent. When $k=\mathbb C$, our anti-tempered parameters exactly coincide with the special unipotent parameters defined in \cite{BarbaschVogan1985}. When $k=\mathbb R$, they are a (proper) subset of the special unipotent parameters considered in \cite[\S27]{AdamsBarbaschVogan}. When $k$ is $p$-adic, there may be other types of parameters which deserve the label of `unipotent'. For example, it may be reasonable to call `unipotent' any Arthur parameter which is trivial when restricted to the inertia subgroup $I_k$. Thankfully, our aim in this paper is \emph{not} to resolve the debate regarding the definition of `unipotent', but rather to construct some interesting Arthur packets (which are unambiguously unipotent). As we will explain in section \ref{sec:duality}, our proposed definition of anti-tempered Arthur packets is consistent, a posteriori, with the `dual-tempered' packets defined in \cite[(7.1.9),(7.1.10)]{Arthur2013}. 

Of course, it is very easy to parameterize the set of anti-tempered parameters. 
By the Jacobson-Morozov theorem, there is a natural bijection
%
\begin{align*}
\{\text{nilpotent adjoint } G^{\vee}\text{-orbits}\} &\xrightarrow{\sim} \{\text{anti-tempered Arthur parameters}\}/G^{\vee}\\
\OO^{\vee} &\mapsto \psi_{\OO^{\vee}}.
\end{align*}
%
To simplify the notation, we write $\Pi^{\mathsf{Art}}_{\OO^{\vee}}(\mathbf{G}(k)) := \Pi^{\mathsf{Art}}_{\psi_{\OO^{\vee}}}(\mathbf{G}(k))$. 

In Section \ref{sec:results} we will propose a definition of $\Pi^{\mathsf{Art}}_{\OO^{\vee}}(\mathbf{G}(k))$ for every nilpotent adjoint $G^{\vee}$-orbit $\OO^{\vee}$. Our approach in this paper closely follows \cite{BarbaschVogan1985}, where a similar problem was solved for \emph{complex} reductive groups. Before giving our definition, we review the main results of \cite{BarbaschVogan1985} so the connection is clear.



\subsection{Complex groups}\label{subsec:complexgroups}

Let $G$ be a complex connected reductive algebraic group. For $\lambda \in \mathfrak{h}^*/W$, write $\Pi_{\lambda}(G)$ for the (finite) set of (equivalence classes of) irreducible $G$-representations with left and right infinitesimal character $\lambda$. For an irreducible $G$-representation $X$, write $\WF(X) \subset \cN$ for the (unique) open $G$-orbit in the wavefront set of $X$. 

Fix an even nilpotent orbit $\OO^{\vee} \subset \cN^{\vee}$. Choose an $\mathfrak{sl}(2)$-triple $(e^{\vee},f^{\vee},h^{\vee})$ with $e^{\vee} \in \OO^{\vee}$. Let $d: \cN^{\vee}_o \to \cN_o$ denote the duality map defined by Spaltenstein in \cite[Proposition 10.3]{Spaltenstein} (see also \cite[\S13.3]{Lusztig1984} and \cite[Appendix A]{BarbaschVogan1985}). The first main result in \cite{BarbaschVogan1985} is a lower bound on the wavefront sets of certain irreducible representations. 

\begin{theorem}[Corollary 5.18, \cite{BarbaschVogan1985}]\label{thm:WFBV}
Suppose $X \in \Pi_{\frac{1}{2}h^{\vee}}(G)$. Then
%
$$d(\OO^{\vee}) \leq \WF(X).$$
%
%where $d$ denotes the Barbasch-Vogan duality map.
\end{theorem}

One of the main contributions of \cite{BarbaschVogan1985} is a definition of the unipotent Arthur packet $\Pi_{\OO^{\vee}}^{\mathsf{Art}}(G)$.

\begin{definition}[Definition 1.17, \cite{BarbaschVogan1985}]\label{def:unipotentBV}
The unipotent Arthur packet attached to $\OO^{\vee}$ is the set
%
$$\Pi^{\mathsf{Art}}_{\OO^{\vee}}(G) := \{X \in \Pi_{\frac{1}{2}h^{\vee}}(G) \mid \WF(X) \leq d(\OO^{\vee})\}$$
\end{definition}

\begin{rmk}
For $X \in \Pi_{\frac{1}{2}h^{\vee}}(G)$, we have $d(\OO^{\vee}) \leq \WF(X)$ by Theorem \ref{thm:WFBV}. So the condition $\WF(X) \leq d(\OO^{\vee})$ is equivalent to the requirement $\WF(X) = d(\OO^{\vee})$.
\end{rmk}

Also in \cite{BarbaschVogan1985} is a parameterization of $\Pi^{\mathsf{Art}}_{\OO^{\vee}}(G)$. Write $A(\OO^{\vee})$ for the $G^{\vee}$-equivariant fundamental group of $\OO^{\vee}$ and $\bar{A}(\OO^{\vee})$ for Lusztig's canonical quotient \cite[\S13.1]{Lusztig1984}, \cite[\S5]{Sommers2001}. 

\begin{theorem}[Theorem III, \cite{BarbaschVogan1985}]\label{thm:classificationBV}
There is a natural bijection
%
$$\mathrm{Irr}(\bar{A}(\OO^{\vee})) \xrightarrow{\sim} \Pi^{\mathsf{Art}}_{\OO^{\vee}}(G)$$
\end{theorem}

If we drop the requirement that $\OO^{\vee}$ is even, Theorems \ref{thm:WFBV} and \ref{thm:classificationBV} hold word-for-word. The more general statements are proved (by rather different methods) in \cite{LMBM}.




\subsection{Anti-tempered Arthur packets and weak Arthur packets}

Motivated by (2) of Theorem \ref{t:main}, we define the Arthur packet attached to the anti-tempered parameter $\psi_{\OO^{\vee}}$
%
\begin{equation}\label{eq:defofpacket}\Pi^{\mathsf{Art}}_{\OO^\vee}(\bfG(\mathsf k)) := \{X=X(q^{\frac 12 h^\vee},n,\rho) \mid  \ ^K\WF(X) \leq_A D(\OO^{\vee},1)\}.\end{equation}
%
This is our analog of Definition \ref{def:unipotentBV}. Our main result on Arthur packets is the following.

\begin{theorem}[See Theorem \ref{thm:antitempered} below]\label{thm:antitempered-main}
Suppose $X=X(q^{\frac 12 h^\vee},n,\rho)$ is an irreducible Iwahori-spherical representation. Then $X$ belongs to $\Pi^{\mathsf{Art}}_{\OO^\vee}(\bfG(\mathsf k))$ if and only if
$\AZ(X)$ is tempered. In particular, the Iwahori-spherical representations in $\Pi^{\mathsf{Art}}_{\OO^\vee}(\bfG(\mathsf k))$ are
\begin{enumerate}
\item unitary;
\item in bijection with the set
\[ \mathrm{Irr}(A(\OO^{\vee}))_0=\{\rho\in \mathrm{Irr}(A(\OO^{\vee}))\mid \rho\text{ of Springer type}\}.
\]
\end{enumerate}
\end{theorem}
%Here, $\rho \in \mathrm{Irr}(A(\OO^{\vee}))$ is of `Springer type' if it corresponds under the Springer correspondence to an irreducible $W$-representation\todo{we defined springer type above}. 
The unitarity in (1) follows from a result of Barbasch and Moy, see Section \ref{sec:AZduality}. If we drop the condition that $X$ is Iwahori-spherical, we expect Theorem \ref{thm:antitempered-main} to remain true, so that
%
$$\mathrm{Irr}(A(\OO^{\vee})) \xrightarrow{\sim} \Pi_{\OO^{\vee}}^{\mathsf{Art}}(\mathbf{G}(\sfk)).$$
%
This is our analog of Theorem \ref{thm:classificationBV}. We note that in particular, our result says that Jiang's conjecture \cite[Conjecture 1.6]{LiuShahidi} holds for the anti-tempered Arthur packets $\psi_{\OO^\vee}$ (or at least for their Iwahori constituents). 

\medskip

Importantly, if we had used the condition $^{\bark}\WF(X) \leq d(\OO^{\vee})$, instead of the condition $^K\WF(X) \leq_A D(\OO^{\vee},1)$, to define the Arthur packet $\Pi^{\mathsf{Art}}_{\OO^\vee}(\bfG(\mathsf k))$, Theorem \ref{thm:antitempered-main} would no longer hold. %(for further discussion of this point, see Sections \ref{sec:duality} and \ref{sec:example} below).

Instead, this leads us to the notion of \emph{weak Arthur packets}. Our definition (\ref{eq:defofpacket}) of the Arthur packet $\Pi^{\mathsf{Art}}_{\OO^\vee}(\bfG(\mathsf k))$ attached to $\OO^{\vee}$ is stated in terms of the {canonical unramified wavefront set} $^K\WF(X)$. If we replace $^K\WF(X)$ with the coarser invariant $\hphantom{ }^{\bar{\sfk}}\WF(X)$, we get a set
%
\begin{equation}\label{eq:weakpacket}
\Pi_{\OO^{\vee}}^{\mathsf{Weak}}(\mathbf{G}(\sfk)) := \{X = X(q^{\frac{1}{2}h^{\vee}},n,\rho) \mid \hphantom{ }^{\bar{\sfk}}\WF(X) \leq d(\OO^{\vee})\}.
\end{equation}
%
Because of the compatibility between $^K\WF(X)$ and $\hphantom{ }^{\bar{\sfk}}\WF(X)$, there is a containment
%
$$\Pi_{\OO^{\vee}}^{\mathsf{Art}}(\mathbf{G}(\sfk)) \subseteq \Pi_{\OO^{\vee}}^{\mathsf{Weak}}(\mathbf{G}(\sfk)).$$
%
In contrast to the set $\Pi^{\mathsf{Art}}_{\OO^\vee}(\bfG(\mathsf k))$, the set $\Pi_{\OO^{\vee}}^{\mathsf{Weak}}(\mathbf{G}(\sfk))$ is \emph{not} the $\AZ$-dual of a tempered Arthur packet, nor is it parameterized (in any simple way) via representations of $A(\OO^{\vee})$. So it is not a reasonable candidate for an Arthur packet. By analogy with the case of real reductive groups (see \cite[Chapter 27]{AdamsBarbaschVogan}), we call $\Pi_{\OO^{\vee}}^{\mathsf{Weak}}(\mathbf{G}(\sfk))$ the \emph{weak Arthur packet} attached to $\OO^{\vee}$. 

{As a consequence of Theorem \ref{t:main}, it is easy to describe the Iwahori constituents of $\Pi_{\OO^{\vee}}^{\mathsf{Weak}}(\mathbf{G}(\sfk))$ as follows.

\begin{cor}\label{c:weak} An irreducible Iwahori-spherical representation belongs to 
$\Pi_{\OO^{\vee}}^{\mathsf{Weak}}(\mathbf{G}(\sfk))$ if and only if it is of the form $\mathsf{AZ}(X(q^{\frac{1}{2}h^{\vee}},n,\rho))$, where $n$ belongs to the special piece (in the sense of \cite{Spaltenstein}) of $\OO^\vee.$
\end{cor}
}

\begin{conj}\label{conj:weakpacket}
The set $\Pi_{\OO^{\vee}}^{\mathsf{Weak}}(\mathbf{G}(\sfk))$ is a (possibly non-disjoint) union of several Arthur packets 
%
\begin{equation}\label{eq:unionpackets}\Pi_{\OO^{\vee}}^{\mathsf{Weak}}(\mathbf{G}(\sfk)) = \bigcup_{i=1}^n \Pi_{\widetilde{\psi}_i}^{\mathsf{Art}}(\mathbf{G}(\sfk)),\end{equation}
%
corresponding to a collection of simplified Arthur parameters %(each trivial on the Weil group $W_k$)
%
\begin{equation}\{\widetilde{\psi}_i: W_{\mathsf k} \times \mathrm{SL}(2,\CC)_{\mathsf{Lan}} \times \mathrm{SL}(2,\CC)_{\mathsf{Art}} \to G^{\vee} \mid \ 1 \leq i \leq n\},\end{equation}
%
including the anti-tempered parameter $\widetilde{\psi}_{\OO^{\vee}}$, but also several others. Each $\widetilde{\psi}_i$ is trivial on the Weil group $W_k$ and thus corresponds to an algebraic homomorphism
%
$$\widetilde{\psi}_i: \mathrm{SL}(2,\CC)_{\mathrm{Lan}} \times \mathrm{SL}(2,\CC)_{\mathsf{Art}} \to G^{\vee}$$
%
Via the Jacobson-Morozov theorem, each such $\widetilde{\psi}_i$ can be identified with a pair of nilpotent adjoint $G^{\vee}$-orbits
%
\begin{equation}\label{eq:commutingorbits}(\OO^{\vee}_{i,\mathsf{Art}},\OO^{\vee}_{i,\mathsf{Lan}}),\end{equation}
%
and a pair of semisimple elements in a single fixed Cartan subalgebra of $\fg^{\vee}$
%
\begin{equation}\label{eq:commuting semisimple}(h^{\vee}_{i,\mathsf{Art}}, h^{\vee}_{i,\mathsf{Lan}}).\end{equation}
%
These elements should satisfy
%
\begin{equation}\label{eq:inflcharsum}\frac{1}{2}h^{\vee} \in G^{\vee}(\frac{1}{2}h^{\vee}_{i,\mathsf{Art}} + \frac{1}{2}h^{\vee}_{i,\mathsf{Lan}}).\end{equation}
\end{conj}

One might be tempted to guess that the set $\{\widetilde{\psi}_i\}$ of parameters appearing in Conjecture \ref{conj:weakpacket} consists of \emph{all} possible parameters satisfying the infinitesimal character condition (\ref{eq:inflcharsum}). But nothing quite so simple is true. The tempered Arthur packet 
corresponding to the pair $(\OO^{\vee}_{\mathsf{Art}},\OO^{\vee}_{\mathsf{Lan}}) = (0, \OO^{\vee})$ is almost never contained in $\Pi_{\OO^{\vee}}^{\mathsf{Weak}}(\mathbf{G}(\sfk))$ (see Section \ref{sec:example} for a detailed example). Thus, the problem of describing the Arthur packets in $\Pi_{\OO^{\vee}}^{\mathsf{Weak}}(\mathbf{G}(\sfk))$ seems interesting and nontrivial. {We mention that Conjecture \ref{conj:weakpacket} together with Corollary \ref{c:weak} imply the following conjecture (noting that $\mathsf{AZ}$ preserves unitarity):
\begin{conj}
For all nilpotent elements $n$ in the special piece of $\OO^\vee$, the representations $X(q^{\frac 12 h^\vee},n,\rho)$ are unitary.
\end{conj}
}






\subsection{Duality}\label{sec:duality} 

We conclude by offering some evidence in favor of our proposed definition (\ref{eq:defofpacket}) of the unipotent Arthur packet $\Pi_{\OO^{\vee}}^{\mathsf{Art}}(\mathbf{G}(\sfk))$, using the two criteria  stated in Conjecture \ref{conj:Arthur}. For $\psi = \psi_{\OO^{\vee}}$ an anti-tempered parameter, the corresponding Langlands packet $\Pi_{\phi_{\psi}}^{\mathsf{Lan}}(\mathbf{G}(\sfk))$ is a singleton consisting of the spherical Arthur representation. This representation is contained in our proposed Arthur packet $\Pi_{\OO^{\vee}}^{\mathsf{Art}}(\mathbf{G}(\sfk))$ by the main result of \cite{okada2021wavefront}. The second criterion of Conjecture \ref{conj:Arthur} follows from (1) of Theorem \ref{thm:antitempered-main}. 

For $p$-adic groups, there is an an additional condition that Arthur packets should satisfy. To formulate it, it will be convenient to recall an alternative formulation of the Langlands classification. A \emph{simplified Langlands parameter} is a continuous homomorphism $\widetilde{\varphi}: W_{\sfk} \times \mathrm{SL}(2,\CC) \to G^{\vee}$ such that $\widetilde{\varphi}(W_k)$ consists of semisimple elements and $\widetilde{\varphi}|_{\mathrm{SL}(2,\CC)}$ is algebraic. A simplified Langlands parameter is tempered if the image of $W_k$ is compact (the idea of replacing the Weil-Deligne group $W_k'$ with $W_k \times \mathrm{SL}(2,\CC)$ in the non-Archimedean case was first proposed by Langlands in \cite[p. 209]{Langlands1979}). Although there are good reasons for preferring the Weil-Deligne group formulation, there is a bijection between simplified and honest Langlands parameters, see \cite[p. 278]{Knapp-Langlands}. Similarly, a \emph{simplified Arthur parameter} is a continuous homomorphism $\widetilde{\psi}: W_k \times \mathrm{SL}(2,\CC)_{\mathsf{Lan}} \times \mathrm{SL}(2,\CC)_{\mathsf{Art}} \to G^{\vee}$ such that the restriction of $\widetilde{\psi}$ to $W_k \times \mathrm{SL}(2,\CC)_{\mathsf{Lan}}$ is a tempered simplified Langlands parameter and the restriction of $\widetilde{\psi}$ to $\mathrm{SL}(2,\CC)_{\mathsf{Art}}$ is algebraic. The bijection between simplified and honest Langlands parameters induces a bijection between simplified and honest Arthur parameters. 

If $\widetilde{\psi}$ is a simplified Arthur parameter, we get a second simplified Arthur parameter $\widetilde\psi^t$ by `flipping' the $\mathrm{SL}(2,\CC)$ factors, \cite[p. 390]{Arthur2013}, i.e.
%
$$\widetilde\psi^t(w,x,y) :=\widetilde \psi(w,y,x),  \qquad w \in W_k, \ x,y \in \mathrm{SL}(2,\CC).$$
%
Via the bijection between simplified and honest Arthur parameters, the map $\widetilde{\psi} \mapsto \widetilde{\psi}^t$ induces an involution on honest Arthur parameters, which we also denote by $\psi \mapsto \psi^t$. It is expected that
%
\begin{equation}\label{eq:AZflip}\mathsf{AZ}(\Pi_{\psi}^{\mathsf{Art}}(\mathbf{G}(\mathsf{k}))) = \Pi_{\psi^t}^{\mathsf{Art}}(\mathbf{G}(\mathsf{k})).\end{equation}
%
In the case when $\mathbf G$ is orthogonal or symplectic, this duality is discussed in \cite[\S7.1]{Arthur2013}. If the Arthur parameter $\psi$ is trivial on the inertia subgroup $I_k$, then the associated Langlands parameter $\phi_{\psi}$ is unramified. So the representations in the Langlands packet $\Pi_{\phi_{\psi}}^{\mathsf{Lan}}(\mathbf{G}(\sfk))$, and hence also in the Arthur packet $\Pi_{\psi}^{\mathsf{Art}}(\mathbf{G}(\mathsf{k}))$, are of unipotent cuspidal support. If $\widetilde\psi$ is trivial on $W_k \times \SL(2,\CC)_{\mathsf{Art}}$, then $\Pi_{\psi}^{\mathsf{Art}}(\mathbf{G}(\sfk)) = \Pi_{\phi_{\psi}}^{\mathsf{Lan}}(\mathbf{G}(\sfk))$ consists of \emph{tempered} representations with real infinitesimal character. So if $\psi$ is anti-tempered (cf. Definition \ref{def:unipotentparam}), our additional desideratum (\ref{eq:AZflip}) suggests that $\AZ(\Pi_{\psi}^{\mathsf{Art}}(\mathbf{G}(\sfk)))$ is tempered. This is consistent with Theorem \ref{thm:antitempered-main}. 

In \cite[(7.1.10)]{Arthur1983}, it is proved that the Arthur packets corresponding to simplified Arthur parameters with trivial restriction to $\SL(2,\CC)_{\mathsf{Lan}}$ are the $\AZ$-duals of the tempered $L$-packets, as defined in \cite[Theorem 1.5.1]{Arthur1983}. It is expected that the tempered Deligne-Langlands-Lusztig $L$-packets coincide with Arthur's unramified tempered $L$-packets, but this has been verified only in the case when $\bfG=\mathrm{SO}(2n+1)$, see \cite[Th\'eor\`eme, p.463]{MW2003}, \cite[Th\'eor\`eme, p.89]{Wald-endoscopy}. For the general case what is missing is a verification of the properties of stability and endoscopic transfer for tempered Deligne-Langlands-Lusztig $L$-packets.


